Non-Perturbative Lepton Sea Fermions in the Nucleon and the Proton Radius Puzzle

A potential explanation [U.~D.~Jentschura, Phys.\ Rev.\ A {\bf 88}, 062514 (2013)] of the proton radius puzzle originating from the non-perturbative lepton-pair content of the proton is studied. Well-defined quantities that depend on this lepton-pair content are evaluated. Each is found to be of the order of $10({\alpha\over \pi})^2$, so that we find such a lepton-pair content exists in the proton. However, we argue that this relatively large result and general features of loop diagrams rule out the possibility of lepton-pair content as an explanation of the proton radius puzzle. In addition, the contributions of a class of explanations of the proton radius puzzle (for which the dependence on the $\mu p$ relative distance is as a contact interaction) is determined.

==> texdefinitions <==
%\parindent=0pt
%\addtolength{\textheight}{0mm}
%\textheight=268 mm
%\topmargin=-28 mm
%\oddsidemargin=12.0mm
%\textwidth=141 mm

%\setcounter{secnumdepth}{3}
%\setcounter{tocdepth}{3}

%\usepackage{epsfig}
%\usepackage[named]{color}
%\RequirePackage{nicefrac}

\usepackage{amsmath,amssymb,amsfonts,graphicx,makeidx,fancybox}
\usepackage{xcolor}
\usepackage{dcolumn}
\usepackage{multirow}
\usepackage{ulem}
\usepackage[caption=false]{subfig}
\usepackage{wrapfig}

\RequirePackage{cancel}    % useful for Feynman slash notation
\RequirePackage{slashed}   % also for slash notation: take your pick!

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\a{\alpha}
\def\b{\beta}
\def\d{\delta}
\def\g{\gamma}
\def\e{\epsilon}
\def\ve{\varepsilon}
\def\vp{\varphi}
\def\z{\zeta}
\def\th{\theta}
\def\k{\kappa}
\def\l{\lambda}
\def\s{\sigma}
\def\o{\omega}

\def\D{\Delta}
\def\G{\Gamma}
\def\L{\Lambda}
\def\O{\Omega}
\def\S{\Sigma}
\def\T{\Theta}

\def\pl{\partial}
\def\hs{\hspace}
\def\ms{\mspace}
\def\ol{\overline}
\def\no{\nonumber}
\def\ni{\noindent}

\def\ua{\uparrow}
\def\da{\downarrow}
\def\para{\parallel}

\def\lf{\left}
\def\rg{\right}
\def\la{\langle}
\def\ra{\rangle}
\def\lv{\lvert}
\def\rv{\rvert}
\def\lV{\lVert}
\def\rV{\rVert}

\def\lra{\longrightarrow}
\def\Lra{\Longrightarrow}
\def\lla{\longleftarrow}
\def\Lla{\Longleftarrow}
\def\Llra{\Longleftrightarrow}


\def\qqquad{\qquad\quad}
\def\qqqquad{\qquad\qquad}

\newcommand{\vect}[1]{\boldsymbol{#1}}
\newcommand{\ph}[1]{\phantom{#1}}

%\newcommand{\ss}[1]{\scriptstyle{#1}}
\newcommand{\sss}[1]{\scriptscriptstyle{#1}}


\definecolor{darkgreen}{cmyk}{1,0,1,0.5}
\definecolor{darkblue}{cmyk}{0.777,0.777,0,0.561}
\definecolor{heavyred}{rgb}{.750,0.00,0.00}

\newcommand{\dgreen}{\textcolor{darkgreen}}
\newcommand{\dblue}{\textcolor{darkblue}}
\newcommand{\hred}{\textcolor{heavyred}}



\newcommand{\Apricot}        {\textcolor{Apricot}}
\newcommand{\Aquamarine}     {\textcolor{Aquamarine}}
\newcommand{\Bittersweet}    {\textcolor{Bittersweet}}
\newcommand{\Black}          {\textcolor{Black}}
\newcommand{\Blue}           {\textcolor{Blue}}
\newcommand{\BlueGreen}      {\textcolor{BlueGreen}}
\newcommand{\BlueViolet}     {\textcolor{BlueViolet}}
\newcommand{\BrickRed}       {\textcolor{BrickRed}}
\newcommand{\Brown}          {\textcolor{Brown}}
\newcommand{\BurntOrange}    {\textcolor{BurntOrange}}
\newcommand{\CadetBlue}      {\textcolor{CadetBlue}}
\newcommand{\CarnationPink}  {\textcolor{CarnationPink}}
\newcommand{\Cerulean}       {\textcolor{Cerulean}}
\newcommand{\CornflowerBlue} {\textcolor{CornflowerBlue}}
\newcommand{\Cyan}           {\textcolor{Cyan}}
\newcommand{\Dandelion}      {\textcolor{Dandelion}}
\newcommand{\DarkOrchid}     {\textcolor{DarkOrchid}}
\newcommand{\Emerald}        {\textcolor{Emerald}}
\newcommand{\ForestGreen}    {\textcolor{ForestGreen}}
\newcommand{\Fuchsia}        {\textcolor{Fuchsia}}
\newcommand{\Goldenrod}      {\textcolor{Goldenrod}}
\newcommand{\Gray}           {\textcolor{Gray}}
\newcommand{\Green}          {\textcolor{Green}}
\newcommand{\GreenYellow}    {\textcolor{GreenYellow}}
\newcommand{\JungleGreen}    {\textcolor{JungleGreen}}
\newcommand{\Lavender}       {\textcolor{Lavender}}
\newcommand{\LimeGreen}      {\textcolor{LimeGreen}}
\newcommand{\Magenta}        {\textcolor{Magenta}}
\newcommand{\Mahogany}       {\textcolor{Mahogany}}
\newcommand{\Maroon}         {\textcolor{Maroon}}
\newcommand{\Melon}          {\textcolor{Melon}}
\newcommand{\MidnightBlue}   {\textcolor{MidnightBlue}}
\newcommand{\Mulberry}       {\textcolor{Mulberry}}
\newcommand{\NavyBlue}       {\textcolor{NavyBlue}}
\newcommand{\OliveGreen}     {\textcolor{OliveGreen}}
\newcommand{\Orange}         {\textcolor{Orange}}
\newcommand{\OrangeRed}      {\textcolor{OrangeRed}}
\newcommand{\Orchid}         {\textcolor{Orchid}}
\newcommand{\Peach}          {\textcolor{Peach}}
\newcommand{\Periwinkle}     {\textcolor{Periwinkle}}
\newcommand{\PineGreen}      {\textcolor{PineGreen}}
\newcommand{\Plum}           {\textcolor{Plum}}
\newcommand{\ProcessBlue}    {\textcolor{ProcessBlue}}
\newcommand{\Purple}         {\textcolor{Purple}}
\newcommand{\RawSienna}      {\textcolor{RawSienna}}
\newcommand{\Red}            {\textcolor{Red}}
\newcommand{\RedOrange}      {\textcolor{RedOrange}}
\newcommand{\RedViolet}      {\textcolor{RedViolet}}
\newcommand{\Rhodamine}      {\textcolor{Rhodamine}}
\newcommand{\RoyalBlue}      {\textcolor{RoyalBlue}}
\newcommand{\RoyalPurple}    {\textcolor{RoyalPurple}}
\newcommand{\RubineRed}      {\textcolor{RubineRed}}
\newcommand{\Salmon}         {\textcolor{Salmon}}
\newcommand{\SeaGreen}       {\textcolor{SeaGreen}}
\newcommand{\Sepia}          {\textcolor{Sepia}}
\newcommand{\SkyBlue}        {\textcolor{SkyBlue}}
\newcommand{\SpringGreen}    {\textcolor{SpringGreen}}
\newcommand{\Tan}            {\textcolor{Tan}}
\newcommand{\TealBlue}       {\textcolor{TealBlue}}
\newcommand{\Thistle}        {\textcolor{Thistle}}
\newcommand{\Turquoise}      {\textcolor{Turquoise}}
\newcommand{\Violet}         {\textcolor{Violet}}
\newcommand{\VioletRed}      {\textcolor{VioletRed}}
\newcommand{\White}          {\textcolor{White}}
\newcommand{\WildStrawberry} {\textcolor{WildStrawberry}}
\newcommand{\Yellow}         {\textcolor{Yellow}}
\newcommand{\YellowGreen}    {\textcolor{YellowGreen}}
\newcommand{\YellowOrange}   {\textcolor{YellowOrange}}




%\def\slantfrac#1#2{\mbox{$\,^#1\!/_#2$}}
%\def\slantfracb#1#2{\mbox{$^#1$}\raisebox{0.8pt}{\mbox{\!\!$\scriptstyle{\not}$}}\,\,\mbox{$_#2$}}
%\def\slantfracc#1#2{\raisebox{-0.3pt}{\mbox{$^#1$}}\raisebox{0.8pt}{\mbox{\!\!$\scriptstyle{\not}$}}\,\,\raisebox{0.3pt}{\mbox{$_#2$}}}
%\def\slantfrac#1#2{\raisebox{-0.5pt}{\mbox{$^#1$}}\raisebox{1.0pt}{\!\mbox{$\scriptstyle{/}$}}\raisebox{0.7pt}{\hs{-0.6pt}\mbox{$_#2$}}}

% define a slanted fraction:
\def\slantfrac#1#2{\kern.1em^{#1}\kern-.3em/\kern-.1em_{#2}}


% Dirac slash
\newcommand{\sh}[1]{\slashed{#1}}

% FONTS
\def\ss{\scriptstyle}
\def\sss{\scriptscriptstyle}


\def\td{\tilde}
\def\+{\text{\raisebox{0.3ex}{$\scriptstyle +$}}}
\def\-{\text{\raisebox{0.3ex}{$\scriptstyle -$}}}

\newcommand{\op}[1]{\boldsymbol{\mathit{#1}}}



\font\bb=bbmss10 scaled 1200
\def\ident{\mbox{\bb 1}}


% AN ENVIRONMENT THAT PLACES A BOX AROUND EVERYTHING
\newenvironment{ibox}[1]%
{\vskip 1.0em
\framebox[\columnwidth][r]{%
\begin{minipage}[c]{\columnwidth}%
\vspace{-1.0em}%
#1%
\end{minipage}}}
%{\vskip 1.0em}


% % A COMMAND THAT PLACES A BOX AROUND EVERYTHING
% \newcommand{\iboxed}[1]{%
% %\setlength{\eqlength}{\textwidth}%
% %\addtolength{\mylength}{\parindent}%
% \vskip 1.0em
% \framebox[\columnwidth][l]{%
% \begin{minipage}[c]{\columnwidth}%
% \vspace{-1.0em}
% #1%
% \end{minipage}}
% \vskip 1.0em}

\newcommand{\iboxed}[1]{%
\vskip 1.0em
\noindent\framebox[\columnwidth][r]{%
\begin{minipage}[c]{\columnwidth}%
\vspace{-1.0em}
#1%
\end{minipage}}
\\[1.0em]}




% A COMMAND THAT PLACES A BOX AROUND EVERYTHING of length 0.8\columnwidth
\newcommand{\iboxedc}[1]{%
\vskip 1.0em
\framebox[0.95\columnwidth][r]{%
\begin{minipage}[c]{\columnwidth}%
\vspace{-1.0em}
#1%
\end{minipage}}
\vskip 1.0em}



% A COMMAND THAT CREATES A BOX STARTING ON RIGHT MARGIN
% MOVING LEFT OF LENGTH #1
\newcommand{\fitbox}[2]{%
\vskip 1.0em
\begin{flushright}
\framebox[{#1}][r]{%
\begin{minipage}[c]{\columnwidth}%
\vspace{-1.0em}
#2%
\end{minipage}}
\end{flushright}
\vskip 1.0em}

% A COMMAND THAT PLACE A BOX AROUND MULTLINE EQUATION c.f. \boxed
\newcommand{\iboxeds}[1]{%
\vskip 1.0em
\begin{equation}
\fbox{%
\begin{minipage}[c]{1mm}%
\vspace{-1.0em}
#1%
\end{minipage}}
\end{equation}
\vskip 1.0em}

\newcommand{\boxedeqn}[1]{%
  \[\fbox{%
      \addtolength{\linewidth}{-2\fboxsep}%
      \addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{\linewidth}%
      \begin{equation}#1\end{equation}%
      \end{minipage}%
    }\]%
}

\newlength{\nl}
\newcommand{\iol}[1]{%
\settowidth{\nl}{$#1$}%
\shortstack{\rule{0.8\nl}{0.05ex}\\[-0.42ex]$\!#1$}}



%\be
%\iol{\a} \ \iol{\b} \ \iol{\g} \ \iol{\d} \ \iol{\e} \ \iol{\ve} \ \iol{\z} \ \iol{\th} \ \iol{k} \ \iol{\l} \ \iol{s} \ \iol{o}
%\quad \iol{\D} \ \iol{\G} \ \iol{\L} \ \iol{\O} \ \iol{\S}
%\quad \iol{A} \ \iol{B} \ \iol{C} \ \iol{D} \ \iol{E} \ \iol{F} \ \iol{G} \ \iol{H} \ \iol{I} \ \iol{J} \
%\iol{K} \ \iol{L} \ \iol{M} \ \iol{N} \ \iol{O} \ \iol{P} \ \iol{Q} \ \iol{R} \ \iol{S} \ \iol{T} \
%\iol{U} \ \iol{V} \ \iol{W} \ \iol{X} \ \iol{Y} \ \iol{Z}
%\ee
%
%\be
%\ol{\a} \ \ol{\b} \ \ol{\g} \ \ol{\d} \ \ol{\e} \ \ol{\ve} \ \ol{\z} \ \ol{\th} \ \ol{k} \ \ol{\l} \ \ol{s} \ \ol{o}
%\quad \ol{\D} \ \ol{\G} \ \ol{\L} \ \ol{\O} \ \ol{\S}
%\quad \ol{A} \ \ol{B} \ \ol{C} \ \ol{D} \ \ol{E} \ \ol{F} \ \ol{G} \ \ol{H} \ \ol{I} \ \ol{J} \
%\ol{K} \ \ol{L} \ \ol{M} \ \ol{N} \ \ol{O} \ \ol{P} \ \ol{Q} \ \ol{R} \ \ol{S} \ \ol{T} \
%\ol{U} \ \ol{V} \ \ol{W} \ \ol{X} \ \ol{Y} \ \ol{Z}
%\ee


% A command that places a shaded box over everything
\newcommand{\icolorbox}[3]{%
\vskip 0.3em
\colorbox{#1}{%
\begin{minipage}[c]{#2\columnwidth}%
\vspace{-1.0em}
#3%
\end{minipage}}
\vskip 0.3em}


% A command that places a shaded box over everything
\newcommand{\icolorboxF}[3]{%
\vskip 0.0em
\colorbox{#1}{%
\begin{minipage}[c]{#2\columnwidth}%
\vskip -2.0em
#3%
\vskip -2.0em
\end{minipage}}
}

